IRFuzzer: Specialized Fuzzing for LLVM Backend Code Generation

Modern compilers, such as LLVM, are complex pieces of software. Due to their complexity, manual testing is unlikely to suffice, yet formal verification is difficult to scale. End-to-end fuzzing can be used, but it has difficulties in achieving high coverage of some components of LLVM. In this paper, we implement IRFuzzer to investigate the effectiveness of specialized fuzzing of the LLVM compiler backend. We focus on two approaches to improve the fuzzer: guaranteed input validity using constrained mutations and improved feedback quality. The mutator in IRFuzzer is capable of generating a wide range of LLVM IR inputs, including structured control flow, vector types, and function definitions. The system instruments coding patterns in the compiler to monitor the execution status of instruction selection. The instrumentation not only provides a new coverage feedback called matcher table coverage, but also provides an architecture specific guidance to the mutator. We show that IRFuzzer is more effective than existing fuzzers by fuzzing on 29 mature LLVM backend targets. In the process, we reported 74 confirmed new bugs in LLVM upstream, out of which 49 have been fixed, five have been back ported to LLVM 15, showing that specialized fuzzing provides useful and actionable insights to LLVM developers.

==> evaluation/6_bug_analysis.tex <==
\subsection{Bugs case study}
\label{sec:eval:analysis}

% In this section, we select some bugs to understand the common traits of the bugs we found to answer \textbf{RQ6}.

\subsubsection{Compiler hang}
\label{sec:eval:analysis:hang}

LLVM may execute multiple optimizations repeatedly until a fixed point is reached.
However, this strategy can result in an infinite loop if not applied carefully, such as when one optimization undoes the effects of a previous optimization.
Four of \numHangs{} hangs we found are caused by this problem.

\input{figs/hang.tex}

For example, \autoref{fig:hang} shows a simplified CFG corresponding to the code generated by \irfuzzer{}.
This CFG will cause a compiler hang due to the interaction between two optimization passes.
BB2 in \autoref{fig:hang:a} consists of a \texttt{switch} statement with two self loop edges.
The \texttt{TurnSwitchRangeIntoICmp} optimization attempts to rewrite the condition as a branch predicate because \texttt{x == 2 || x == 3} can be optimized using bit operations, rewriting \autoref{fig:hang:a} into \autoref{fig:hang:b}.
However, the \texttt{FoldValueComparisonIntoPredecessors} optimization converts this code back into a \texttt{switch} statement to reduce the number of comparison operations, turning the CFG back to \autoref{fig:hang:a}.
As a result, a fixed point is never reached, creating an infinite loop.

This bug is hard to trigger since the bug can only be triggered when the \texttt{switch} in \autoref{fig:hang:b} has exactly two destinations (BB2 and BB3), and the switch conditions are consecutive, enabling the \texttt{TurnSwitchRangeIntoICmp} optimization.
This combination is unlikely to be created during manual testing, and can only happen through the interaction of two largely unrelated pieces of code.  Yet, we are able to discover this catastrophic combination through our CFG mutation strategy in a time frame amenable to run fuzzing on every nightly build with little human intervention.

In this case, we answer \textbf{RQ5} by advising the developers to carefully read code that may modify the same location before they push out a new optimization that changes the code.

\subsubsection{Memory error}
\label{sec:eval:analysis:mem}

LLVM often hides memory management from the developers so they don't have to manually manage it.
Still, we found five memory errors: one null pointer dereference, two double frees and two out of bounds (OOB) accesses.
After inspection, we determined that both double free bugs were indirectly caused by OOB accesses, which didn't result in crash immediately.
All four OOB accesses are caused by developers using constants from the program under compilation without validation.
In these cases, an OOB access or undefined behavior in the program being compiled were able to crash the compiler itself.
%It appears that LLVM developers tend to trust that constants in a program are always valid indexes in a data structure, without validating this fact.  Yet, since programs often contain bugs, this assumption can often be incorrect.

As an example, we consider a case involving vector types, shown in \autoref{lst:oob}.
LLVM natively supports to enable SIMD optimizations.
The \texttt{insertelement} \ir{} instruction inserts a value into a vector at a specified index.
If the given index is out of the bounds, the behavior is undefined.
The compiler can leverage this to remove the \texttt{insertelement} instruction.

\begin{comment}
% TODO: Change text bkg color
\begin{lstlisting}[
    float, language=C++, 
    caption={
        A snippet of code in AArch64 where the index (\texttt{IntImm}) is not sanitized before usage.
        This diff is taken between commit \texttt{c635ea5} and \texttt{fb60e50}.
    }, 
    label=lst:oob,
    basicstyle=\ttfamily\scriptsize,
] 
bool CombinerHelper::matchCombineInsertVecElts(...){
  ...
  while (mi_match(
    CurrInst->getOperand(0).getReg(), MRI,
    m_GInsertVecElt(m_MInstr(TmpInst), m_Reg(TmpReg), m_ICst(IntImm)))) 
  {
+  if (IntImm >= NumElts || IntImm < 0)
-  if (IntImm >= NumElts)
    return false;
   if (!MatchInfo[IntImm]) MatchInfo[IntImm] = TmpReg;  (*@\label{lst:oob:oob}@*) 
   CurrInst = TmpInst;
  }
  ...
}
\end{lstlisting}

\begin{lstlisting}[
  float, language=C++, 
  caption={
      A snippet of code in LLVM where index of a vector is treated as signed value.
  }, 
  label=lst:zext,
  basicstyle=\ttfamily\scriptsize,
] 
bool IRTranslator::translateExtractElement(
const User &U, MachineIRBuilder &MIRBuilder)
{ 
Register Idx;
...
const LLT VecIdxTy = LLT::scalar(PreferredVecIdxWidth);
Idx = MIRBuilder.build(*@\textbf{SExt}@*)OrTrunc(VecIdxTy, Idx)
                .getReg(0);
...
}
\end{lstlisting}
\end{comment}

% Figure arrangement for FSE 2024 (Single column)
\begin{figure}[t]
    \begin{minipage}{0.48\linewidth}
        \begin{subfigure}[t]{0.9\linewidth}
            \begin{lstlisting}[
    language=C++, 
    caption={
        A snippet of code in AArch64 where the index (\texttt{IntImm}) is not sanitized before usage.
        This diff is our patch to fix this bug.
    }, 
    label=lst:oob,
    basicstyle=\ttfamily\scriptsize,
] 
bool CombinerHelper::matchCombineInsertVecElts(...){
  while (...) {
+   if (IntImm >= NumElts || IntImm < 0)
-   if (IntImm >= NumElts)
      return false;
    if (!MatchInfo[IntImm]) 
        MatchInfo[IntImm] = TmpReg;  (*@\label{lst:oob:oob}@*) 
    CurrInst = TmpInst;
    ...
  }
}
\end{lstlisting}
        \end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}{0.51\linewidth}
        \begin{subfigure}[t]{0.9\linewidth}
            \begin{lstlisting}[
  language=C++, 
  caption={
      A snippet of code in LLVM where index of a vector is treated as signed value. This diff is our patch to fix this bug.
  }, 
  label=lst:zext,
  basicstyle=\ttfamily\scriptsize,
] 
bool IRTranslator::translateExtractElement(
  const User &U, 
  MachineIRBuilder &MIRBuilder) { 
    Register Idx;
    const LLT VecIdxTy = LLT::scalar(PreferredVecIdxWidth);
    Idx = MIRBuilder
-          .build(*@\textbf{SExt}@*)OrTrunc(VecIdxTy, Idx)
+          .build(*@\textbf{ZExt}@*)OrTrunc(VecIdxTy, Idx)
           .getReg(0);
    ...
}
\end{lstlisting}
        \end{subfigure}
    \end{minipage}
    \caption{
        Two bugs we found in LLVM code base. Both of them will lead to compiler crash and have been fixed.
    }
    % \vspace{-0.5\baselineskip}
    \label{fig:ir}
\end{figure}



%However, in practise, developers may forget to check for the validity and directly access the operand of a vector.
In most cases, LLVM's module verifier checks for invalid indices, and will reject any negative indices before compilation.
As a result, developers may implicitly assume that indices in this code are \textit{always} non-negative.
However, the module verifier does allow \texttt{undef} as a valid index.
\texttt{Undef} in LLVM represents a value is can be anything, and is represented as an index \texttt{IntImm} of $-1$ at this point in the code, resulting in an OOB access at line \autoref{lst:oob:oob}.

This example shows that our \ir{} mutation method is better than high-level language generation, since \texttt{undef} is not a primitive high-level language construct and will only be introduced through other optimizations.
By generating LLVM IR directly, we have more control over instruction operands and can directly generate values like \texttt{undef}.
To answer \textbf{RQ5}, we recommend developers to be careful about uncommon values like \texttt{undef} and \texttt{poison}, which may appear during compilation.

\subsubsection{Logic error}
\label{sec:eval:analysis:logic}

Logic error usually starts with unclear documentation or undocumented assumptions.
Middle-end and backend are developed by different programmers, who may interpret ambiguous documentations differently.

For example, \autoref{lst:zext} shows a bug we found in the LLVM backend.
When translating the \ir{} \texttt{extractelement}, the index is extended as a signed integer.
The code translates constants like \texttt{char 255} into \texttt{-1}.
This bug generates incorrect \mir{s} and affects the LLVM backend for seven architectures.

The bug was introduced in LLVM nine years ago and was never noticed for several reasons.
First, it is less common for compiler frontends to generate vector operations, as we have seen in \autoref{sec:eval:csmith}, and even more rare to use an index that is large enough to wrap around to a negative integer.
However, more importantly, we discovered that the documentation was ambiguous with respect to the desired behavior.
The documentations indicated that ``The index may be a variable of any integer type'' without giving more details on how it should be interpreted.
Therefore, when this bug was introduced nine years ago, it was actually compliant with the incomplete documentation at the time.
This exemplifies how complex software interfaces can be incompletely specified, which further justifies our specialized fuzzing.
In this case, we have fixed the bug and updated the documentation to reflect the intended interpretation of the index as an unsigned integer.
To answer \textbf{RQ5}, we encourage developers of LLVM to communicate more on the documentations. Review and update documentations with the development of the code would be a good practice.

\begin{comment}

\subsubsection{Assertion error}
\label{sec:eval:analysis:assert}

57283

58615

\subsubsection{Missing features}
\label{sec:eval:analysis:features}

59009
\end{comment}
